The crucial role of surface magnetic fields for stellar dynamos: Epsilon Eridani, 61 Cygni A, and the Sun

Cool main-sequence stars, such as the Sun, have magnetic fields which are generated by an internal dynamo mechanism. In the Sun, the dynamo mechanism produces a balance between the amounts of magnetic flux generated and lost over the Sun's 11-year activity cycle and it is visible in the Sun's different atmospheric layers using multi-wavelength observations. We used the same observational diagnostics, spanning several decades, to probe the emergence of magnetic flux on the two close by, active- and low-mass K dwarfs: 61 Cygni A and Epsilon Eridani. Our results show that 61 Cygni A follows the Solar dynamo with a regular cycle at all wavelengths, while Epsilon Eridani represents a more extreme level of the Solar dynamo, while also showing strong Solar-like characteristics. For the first time we show magnetic butterfly diagrams for stars other than the Sun. For the two K stars and the Sun, the rate at which the toroidal field is generated from surface poloidal field is similar to the rate at which toroidal flux is lost through flux emergence. This suggests that the surface field plays a crucial role in the dynamos of all three stars. Finally, for Epsilon Eridani, we show that the two chromospheric cycle periods, of ~3 and ~13 years, correspond to two superimposed magnetic cycles.

==> refs.tex <==
@ARTICLE{1998SoPh..181..237B,
       author = {{Beer}, J{\"u}rg and {Tobias}, Steven and {Weiss}, Nigel},
        title = "{An Active Sun Throughout the Maunder Minimum}",
      journal = {\solphys},
         year = 1998,
        month = jul,
       volume = {181},
       number = {1},
        pages = {237-249},
          doi = {10.1023/A:1005026001784},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998SoPh..181..237B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1994A&A...288..293S,
       author = {{Sokoloff}, D. and {Nesme-Ribes}, E.},
        title = "{The Maunder minimum: a mixed-parity dynamo mode?}",
      journal = {\aap},
     keywords = {Asymmetry, Dynamo Theory, Faculae, Nonlinear Equations, Northern Hemisphere, Solar Magnetic Field, Southern Hemisphere, Spatial Distribution, Sunspots, Data Correlation, Magnetohydrodynamics, Sunspot Cycle, Solar Physics, MHD-SUN: ACTIVITY, MAGNETIC FIELD, DYNAMO},
         year = 1994,
        month = aug,
       volume = {288},
        pages = {293-298},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994A&A...288..293S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2012PNAS..10911928H,
       author = {{Hanasoge}, S.~M. and {Duvall}, T.~L. and {Sreenivasan}, K.~R.},
        title = "{Anomalously weak solar convection}",
      journal = {Proceedings of the National Academy of Science},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = jul,
       volume = {109},
       number = {30},
        pages = {11928-11932},
          doi = {10.1073/pnas.1206570109},
archivePrefix = {arXiv},
       eprint = {1206.3173},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012PNAS..10911928H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013A&A...558A..48B,
       author = {{Beeck}, B. and {Cameron}, R.~H. and {Reiners}, A. and {Sch{\"u}ssler}, M.},
        title = "{Three-dimensional simulations of near-surface convection in main-sequence stars. I. Overall structure}",
      journal = {\aap},
     keywords = {convection, hydrodynamics, stars: late-type, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = oct,
       volume = {558},
          eid = {A48},
        pages = {A48},
          doi = {10.1051/0004-6361/201321343},
archivePrefix = {arXiv},
       eprint = {1308.4874},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...558A..48B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2021PNAS..11822518V,
       author = {{Vasil}, Geoffrey M. and {Julien}, Keith and {Featherstone}, Nicholas A.},
        title = "{Rotation suppresses giant-scale solar convection}",
      journal = {Proceedings of the National Academy of Science},
     keywords = {solar convection, Rossby number, rapid rotation, differential rotation},
         year = 2021,
        month = aug,
       volume = {118},
       number = {31},
          eid = {2022518118},
        pages = {2022518118},
          doi = {10.1073/pnas.2022518118},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021PNAS..11822518V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
      }
@ARTICLE{2021NatAs.tmp..165H,
       author = {{Hotta}, H. and {Kusano}, K.},
        title = "{Solar differential rotation reproduced with high-resolution simulation}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = sep,
          doi = {10.1038/s41550-021-01459-0},
archivePrefix = {arXiv},
       eprint = {2109.06280},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021NatAs.tmp..165H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2014MNRAS.438L..76G,
       author = {{Gastine}, T. and {Yadav}, R.~K. and {Morin}, J. and {Reiners}, A. and {Wicht}, J.},
        title = "{From solar-like to antisolar differential rotation in cool stars}",
      journal = {\mnras},
     keywords = {convection, MHD, turbulence, Sun: rotation, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = feb,
       volume = {438},
       number = {1},
        pages = {L76-L80},
          doi = {10.1093/mnrasl/slt162},
archivePrefix = {arXiv},
       eprint = {1311.3047},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.438L..76G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2016ApJ...824..150G,
       author = {{Giguere}, Matthew J. and {Fischer}, Debra A. and {Zhang}, Cyril X.~Y. and {Matthews}, Jaymie M. and {Cameron}, Chris and {Henry}, Gregory W.},
        title = "{A Combined Spectroscopic and Photometric Stellar Activity Study of Epsilon Eridani}",
      journal = {\apj},
     keywords = {planetary systems, stars: individual: HD 22049, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = jun,
       volume = {824},
       number = {2},
          eid = {150},
        pages = {150},
          doi = {10.3847/0004-637X/824/2/150},
archivePrefix = {arXiv},
       eprint = {1606.08553},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...824..150G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2006ApJ...648..607C,
       author = {{Croll}, Bryce and {Walker}, Gordon A.~H. and {Kuschnig}, Rainer and {Matthews}, Jaymie M. and {Rowe}, Jason F. and {Walker}, Andrew and {Rucinski}, Slavek M. and {Hatzes}, Artie P. and {Cochran}, William D. and {Robb}, Russell M. and {Guenther}, David B. and {Moffat}, Anthony F.~J. and {Sasselov}, Dimitar and {Weiss}, Werner W.},
        title = "{Differential Rotation of ɛ Eridani Detected by MOST}",
      journal = {\apj},
     keywords = {Stars: Planetary Systems, Stars: Activity, stars: individual (ɛ Eri), Stars: Late-Type, Stars: Rotation, Stars: Spots},
         year = 2006,
        month = sep,
       volume = {648},
       number = {1},
        pages = {607-613},
          doi = {10.1086/505792},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...648..607C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2013A&A...560A...4R,
       author = {{Reinhold}, Timo and {Reiners}, Ansgar and {Basri}, Gibor},
        title = "{Rotation and differential rotation of active Kepler stars}",
      journal = {\aap},
     keywords = {stars: activity, stars: rotation, starspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = dec,
       volume = {560},
          eid = {A4},
        pages = {A4},
          doi = {10.1051/0004-6361/201321970},
archivePrefix = {arXiv},
       eprint = {1308.1508},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...560A...4R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1999A&A...344..911K,
       author = {{Kitchatinov}, L.~L. and {R{\"u}diger}, G.},
        title = "{Differential rotation models for late-type dwarfs and giants}",
      journal = {\aap},
     keywords = {STARS: ACTIVITY, STARS: LATE-TYPE, STARS: ROTATION},
         year = 1999,
        month = apr,
       volume = {344},
        pages = {911-917},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999A&A...344..911K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Guedel2009A&ARv..17..309G,
       author = {{G{\"u}del}, Manuel and {Naz{\'e}}, Ya{\"e}l},
        title = "{X-ray spectroscopy of stars}",
      journal = {\aapr},
     keywords = {X-rays: stars, Stars: early-type, Stars: late-type, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2009,
        month = sep,
       volume = {17},
       number = {3},
        pages = {309-408},
          doi = {10.1007/s00159-009-0022-4},
archivePrefix = {arXiv},
       eprint = {0904.3078},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&ARv..17..309G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{See2015MNRAS.453.4301S,
       author = {{See}, V. and {Jardine}, M. and {Vidotto}, A.~A. and {Donati}, J. -F. and {Folsom}, C.~P. and {Boro Saikia}, S. and {Bouvier}, J. and {Fares}, R. and {Gregory}, S.~G. and {Hussain}, G. and {Jeffers}, S.~V. and {Marsden}, S.~C. and {Morin}, J. and {Moutou}, C. and {do Nascimento}, J.~D. and {Petit}, P. and {Ros{\'e}n}, L. and {Waite}, I.~A.},
        title = "{The energy budget of stellar magnetic fields}",
      journal = {\mnras},
     keywords = {techniques: polarimetric, stars: activity, stars: magnetic field, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = nov,
       volume = {453},
       number = {4},
        pages = {4301-4310},
          doi = {10.1093/mnras/stv1925},
archivePrefix = {arXiv},
       eprint = {1508.01403},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.453.4301S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Charbonneau2020LRSP...17....4C,
       author = {{Charbonneau}, Paul},
        title = "{Dynamo models of the solar cycle}",
      journal = {Living Reviews in Solar Physics},
     keywords = {Solar cycle, Solar activity, Dynamo, Magnetic fields},
         year = 2020,
        month = jun,
       volume = {17},
       number = {1},
          eid = {4},
        pages = {4},
          doi = {10.1007/s41116-020-00025-6},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020LRSP...17....4C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@BOOK{Krause1980mfmd.book.....K,
       author = {{Krause}, F. and {Raedler}, K.~H.},
        title = "{Mean-field magnetohydrodynamics and dynamo theory}",
         year = 1980,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980mfmd.book.....K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lehmann2021MNRAS.500.1243L,
       author = {{Lehmann}, L.~T. and {Hussain}, G.~A.~J. and {Vidotto}, A.~A. and {Jardine}, M.~M. and {Mackay}, D.~H.},
        title = "{Identifying solar-like magnetic cycles with Zeeman-Doppler-Imaging}",
      journal = {\mnras},
     keywords = {methods: analytical, stars: activity, stars: magnetic field, stars: solar-type, Sun: activity, Sun: magnetic fields, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = jan,
       volume = {500},
       number = {1},
        pages = {1243-1260},
          doi = {10.1093/mnras/staa3284},
archivePrefix = {arXiv},
       eprint = {2010.10214},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.500.1243L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Reinhold2020Sci...368..518R,
       author = {{Reinhold}, Timo and {Shapiro}, Alexander I. and {Solanki}, Sami K. and {Montet}, Benjamin T. and {Krivova}, Natalie A. and {Cameron}, Robert H. and {Amazo-G{\'o}mez}, Eliana M.},
        title = "{The Sun is less active than other solar-like stars}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = may,
       volume = {368},
       number = {6490},
        pages = {518-521},
          doi = {10.1126/science.aay3821},
archivePrefix = {arXiv},
       eprint = {2005.01401},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020Sci...368..518R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Donati2006MNRAS.370..629D,
       author = {{Donati}, J. -F. and {Howarth}, I.~D. and {Jardine}, M.~M. and {Petit}, P. and {Catala}, C. and {Landstreet}, J.~D. and {Bouret}, J. -C. and {Alecian}, E. and {Barnes}, J.~R. and {Forveille}, T. and {Paletou}, F. and {Manset}, N.},
        title = "{The surprising magnetic topology of {\ensuremath{\tau}} Sco: fossil remnant or dynamo output?}",
      journal = {\mnras},
     keywords = {techniques: polarimetric: stars: early-type: stars: individual: {\ensuremath{\tau}} Sco: stars: magnetic fields: stars: rotation: stars: winds, outflows, techniques: polarimetric, stars: early-type, stars: individual: {\ensuremath{\tau}} Sco, stars: magnetic fields, stars: rotation, stars: winds, Astrophysics},
         year = 2006,
        month = aug,
       volume = {370},
       number = {2},
        pages = {629-644},
          doi = {10.1111/j.1365-2966.2006.10558.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0606156},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.370..629D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Simard2020JSWSC..10....9S,
       author = {{Simard}, Corinne and {Charbonneau}, Paul},
        title = "{Grand Minima in a spherical non-kinematic {\ensuremath{\alpha}}$^{2}${\ensuremath{\Omega}} mean-field dynamo model}",
      journal = {Journal of Space Weather and Space Climate},
     keywords = {Solar cycle, solar dynamo, Grand Minima},
         year = 2020,
        month = jan,
       volume = {10},
          eid = {9},
        pages = {9},
          doi = {10.1051/swsc/2020006},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020JSWSC..10....9S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lockwood2007ApJS..171..260L,
       author = {{Lockwood}, G.~W. and {Skiff}, B.~A. and {Henry}, Gregory W. and {Henry}, Stephen and {Radick}, R.~R. and {Baliunas}, S.~L. and {Donahue}, R.~A. and {Soon}, W.},
        title = "{Patterns of Photometric and Chromospheric Variation among Sun-like Stars: A 20 Year Perspective}",
      journal = {\apjs},
     keywords = {Stars: Activity, Stars: Late-Type, Stars: Variables: Other, Astrophysics},
         year = 2007,
        month = jul,
       volume = {171},
       number = {1},
        pages = {260-303},
          doi = {10.1086/516752},
archivePrefix = {arXiv},
       eprint = {astro-ph/0703408},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJS..171..260L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Suresh2020ApJ...904..138S,
       author = {{Suresh}, A. and {Chatterjee}, S. and {Cordes}, J.~M. and {Bastian}, T.~S. and {Hallinan}, G.},
        title = "{Detection of 2{\textendash}4 GHz Continuum Emission from ɛ Eridani}",
      journal = {\apj},
     keywords = {Stellar coronae, K stars, Radio continuum emission, Stellar atmospheres, 305, 878, 1340, 1584, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = dec,
       volume = {904},
       number = {2},
          eid = {138},
        pages = {138},
          doi = {10.3847/1538-4357/abc004},
archivePrefix = {arXiv},
       eprint = {2010.05929},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...904..138S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Folsom2018MNRAS.474.4956F,
       author = {{Folsom}, C.~P. and {Bouvier}, J. and {Petit}, P. and {L{\`e}bre}, A. and {Amard}, L. and {Palacios}, A. and {Morin}, J. and {Donati}, J. -F. and {Vidotto}, A.~A.},
        title = "{The evolution of surface magnetic fields in young solar-type stars II: the early main sequence (250-650 Myr)}",
      journal = {\mnras},
     keywords = {techniques: polarimetric, stars: formation, stars: imaging, stars: magnetic fields, stars: rotation, stars: solar-type, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = mar,
       volume = {474},
       number = {4},
        pages = {4956-4987},
          doi = {10.1093/mnras/stx3021},
archivePrefix = {arXiv},
       eprint = {1711.08636},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.474.4956F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Strassmeier2009A&ARv..17..251S,
       author = {{Strassmeier}, Klaus G.},
        title = "{Starspots}",
      journal = {\aapr},
     keywords = {Starspots, Stars: activity, Stars: imaging, Sunspots, Magnetic fields, Techniques: polarimetric, Stars: rotation, Exoplanets},
         year = 2009,
        month = sep,
       volume = {17},
       number = {3},
        pages = {251-308},
          doi = {10.1007/s00159-009-0020-6},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&ARv..17..251S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2020A&A...636A...7C,
       author = {{Cameron}, R.~H. and {Sch{\"u}ssler}, M.},
        title = "{Loss of toroidal magnetic flux by emergence of bipolar magnetic regions}",
      journal = {\aap},
     keywords = {Sun: magnetic fields, Sun: activity, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = apr,
       volume = {636},
          eid = {A7},
        pages = {A7},
          doi = {10.1051/0004-6361/201937281},
archivePrefix = {arXiv},
       eprint = {2002.05436},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...636A...7C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Bonanno2002A&A...390.1115B,
       author = {{Bonanno}, A. and {Schlattl}, H. and {Patern{\`o}}, L.},
        title = "{The age of the Sun and the relativistic corrections in the EOS}",
      journal = {\aap},
     keywords = {Sun: interior, Sun: oscillations, equation of state, Astrophysics},
         year = 2002,
        month = aug,
       volume = {390},
        pages = {1115-1118},
          doi = {10.1051/0004-6361:20020749},
archivePrefix = {arXiv},
       eprint = {astro-ph/0204331},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002A&A...390.1115B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Wright2011ApJ...743...48W,
       author = {{Wright}, Nicholas J. and {Drake}, Jeremy J. and {Mamajek}, Eric E. and {Henry}, Gregory W.},
        title = "{The Stellar-activity-Rotation Relationship and the Evolution of Stellar Dynamos}",
      journal = {\apj},
     keywords = {stars: activity, stars: coronae, stars: evolution, stars: late-type, stars: magnetic field, stars: rotation, X-rays: stars, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = dec,
       volume = {743},
       number = {1},
          eid = {48},
        pages = {48},
          doi = {10.1088/0004-637X/743/1/48},
archivePrefix = {arXiv},
       eprint = {1109.4634},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...743...48W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Affer2005A&A...433..647A,
       author = {{Affer}, L. and {Micela}, G. and {Morel}, T. and {Sanz-Forcada}, J. and {Favata}, F.},
        title = "{Spectroscopic determination of photospheric parameters and chemical abundances of 6 K-type stars\^}",
      journal = {\aap},
     keywords = {stars: individual: <ASTROBJ>HD 4628</ASTROBJ>, stars: individual: <ASTROBJ>HD 10780</ASTROBJ>, stars: individual: <ASTROBJ>HD 23249</ASTROBJ> ({\ensuremath{\delta}} Eri), stars: individual: <ASTROBJ>HD 198149</ASTROBJ> ({\ensuremath{\eta}} Cep), stars: individual: <ASTROBJ>HD 201091</ASTROBJ> (61 Cyg A), stars: individual: <ASTROBJ>HD 222404</ASTROBJ> ({\ensuremath{\gamma}} Cep)},
         year = 2005,
        month = apr,
       volume = {433},
       number = {2},
        pages = {647-658},
          doi = {10.1051/0004-6361:20041308},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...433..647A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Marsden2014MNRAS.444.3517M,
       author = {{Marsden}, S.~C. and {Petit}, P. and {Jeffers}, S.~V. and {Morin}, J. and {Fares}, R. and {Reiners}, A. and {do Nascimento}, J. -D. and {Auri{\`e}re}, M. and {Bouvier}, J. and {Carter}, B.~D. and {Catala}, C. and {Dintrans}, B. and {Donati}, J. -F. and {Gastine}, T. and {Jardine}, M. and {Konstantinova-Antova}, R. and {Lanoux}, J. and {Ligni{\`e}res}, F. and {Morgenthaler}, A. and {Ram{\`\i}rez-V{\`e}lez}, J.~C. and {Th{\'e}ado}, S. and {Van Grootel}, V. and {BCool Collaboration}},
        title = "{A BCool magnetic snapshot survey of solar-type stars}",
      journal = {\mnras},
     keywords = {line: profiles, magnetic fields, stars: activity, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = nov,
       volume = {444},
       number = {4},
        pages = {3517-3536},
          doi = {10.1093/mnras/stu1663},
archivePrefix = {arXiv},
       eprint = {1311.3374},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.444.3517M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Kervella2008A&A...491..855K,
       author = {{Kervella}, P. and {Fouqu{\'e}}, P.},
        title = "{The angular sizes of dwarf stars and subgiants. Non-linear surface brightness relations in BVR\_cI$_{c}$ from interferometry}",
      journal = {\aap},
     keywords = {stars: fundamental parameters, techniques: interferometric, Astrophysics},
         year = 2008,
        month = dec,
       volume = {491},
       number = {3},
        pages = {855-858},
          doi = {10.1051/0004-6361:200810317},
archivePrefix = {arXiv},
       eprint = {0809.1732},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...491..855K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Barnes2007ApJ...669.1167B,
       author = {{Barnes}, Sydney A.},
        title = "{Ages for Illustrative Field Stars Using Gyrochronology: Viability, Limitations, and Errors}",
      journal = {\apj},
     keywords = {Galaxy: Open Clusters and Associations: General, Stars: Activity, Stars: Evolution, Stars: Late-Type, Stars: Magnetic Fields, Stars: Rotation, Astrophysics},
         year = 2007,
        month = nov,
       volume = {669},
       number = {2},
        pages = {1167-1189},
          doi = {10.1086/519295},
archivePrefix = {arXiv},
       eprint = {0704.3068},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...669.1167B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Valenti2005ApJS..159..141V,
       author = {{Valenti}, Jeff A. and {Fischer}, Debra A.},
        title = "{Spectroscopic Properties of Cool Stars (SPOCS). I. 1040 F, G, and K Dwarfs from Keck, Lick, and AAT Planet Search Programs}",
      journal = {\apjs},
     keywords = {Catalogs, Stars: Abundances, Stars: Fundamental Parameters, Stars: Late-Type, Techniques: Spectroscopic},
         year = 2005,
        month = jul,
       volume = {159},
       number = {1},
        pages = {141-166},
          doi = {10.1086/430500},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJS..159..141V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Petit2021A&A...648A..55P,
       author = {{Petit}, P. and {Folsom}, C.~P. and {Donati}, J. -F. and {Yu}, L. and {do Nascimento}, J. -D. and {Jeffers}, S.~V. and {Marsden}, S.~C. and {Morin}, J. and {Vidotto}, A.~A.},
        title = "{Multi-instrumental view of magnetic fields and activity of ɛ Eridani with SPIRou, NARVAL, and TESS}",
      journal = {\aap},
     keywords = {stars: activity, stars: solar-type, stars: magnetic field, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = apr,
       volume = {648},
          eid = {A55},
        pages = {A55},
          doi = {10.1051/0004-6361/202040027},
archivePrefix = {arXiv},
       eprint = {2101.02643},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...648A..55P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2005ApJ...620L.123U,
       author = {{Ulrich}, Roger K. and {Boyden}, John E.},
        title = "{The Solar Surface Toroidal Magnetic Field}",
      journal = {\apjl},
     keywords = {Sun: Activity, Sun: Magnetic Fields, Sun: Rotation},
         year = 2005,
        month = feb,
       volume = {620},
       number = {2},
        pages = {L123-L127},
          doi = {10.1086/428724},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...620L.123U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2010ASPC..428..109L,
       author = {{Lo}, L. and {Hoeksema}, J.~T. and {Scherrer}, P.~H.},
        title = "{Three Cycles of the Solar Toroidal Magnetic Field and This Peculiar Minimum}",
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
    booktitle = {SOHO-23: Understanding a Peculiar Solar Minimum},
         year = 2010,
       editor = {{Cranmer}, S.~R. and {Hoeksema}, J.~T. and {Kohl}, J.~L.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {428},
        month = jun,
        pages = {109},
archivePrefix = {arXiv},
       eprint = {1003.3981},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ASPC..428..109L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994SoPh..153..131S,
       author = {{Shrauner}, J.~A. and {Scherrer}, P.~H.},
        title = "{East-west inclination of large-scale photospheric magnetic fields}",
      journal = {\solphys},
     keywords = {Line Spectra, Magnetic Field Configurations, Mathematical Models, Photosphere, Polarity, Solar Cycles, Solar Magnetic Field, Solar Rotation, Iron, Least Squares Method, Magnetic Signatures, Solar Observatories, Solar Physics},
         year = 1994,
        month = aug,
       volume = {153},
       number = {1-2},
        pages = {131-141},
          doi = {10.1007/BF00712496},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994SoPh..153..131S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1979SoPh...61..233D,
       author = {{Duvall}, T.~L., Jr. and {Scherrer}, P.~H. and {Svalgaard}, L. and {Wilcox}, J.~M.},
        title = "{Average photospheric poloidal and toroidal magnetic field components near solar minimum.}",
      journal = {\solphys},
     keywords = {Magnetic Field Configurations, Magnetic Signatures, Photosphere, Solar Magnetic Field, Electric Current, Minima, Solar Wind, Solar Physics, Magnetic Fields:Solar Photosphere, Solar Magnetic Fields:Structure},
         year = 1979,
        month = mar,
       volume = {61},
       number = {2},
        pages = {233-245},
          doi = {10.1007/BF00150408},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1979SoPh...61..233D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1988SoPh..117..291U,
       author = {{Ulrich}, Roger K. and {Boyden}, John E. and {Webster}, Larry and {Snodgrass}, Herschel B. and {Padilla}, Steven P. and {Gilman}, Pamela and {Shieber}, Tom},
        title = "{Solar Rotation Measurements at MT.WILSON - Part Five}",
      journal = {\solphys},
     keywords = {Solar Limb, Solar Magnetic Field, Solar Rotation, Algorithms, Solar Observatories, Solar Oscillations, Solar Physics, Velocity Measurement, Solar Physics},
         year = 1988,
        month = sep,
       volume = {117},
       number = {2},
        pages = {291-328},
          doi = {10.1007/BF00147250},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988SoPh..117..291U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Duncan1991ApJS...76..383D,
       author = {{Duncan}, Douglas K. and {Vaughan}, Arthur H. and {Wilson}, Olin C. and {Preston}, George W. and {Frazer}, James and {Lanning}, Howard and {Misch}, Anthony and {Mueller}, Jean and {Soyumer}, David and {Woodard}, L. and {Baliunas}, Sallie L. and {Noyes}, Robert W. and {Hartmann}, Lee W. and {Porter}, Alain and {Zwaan}, Cornelis and {Middelkoop}, Frans and {Rutten}, Rene G.~M. and {Mihalas}, Dimitri},
        title = "{CA II H and K Measurements Made at Mount Wilson Observatory, 1966--1983}",
      journal = {\apjs},
     keywords = {Stellar Activity, Stellar Composition, Stellar Spectrophotometry, Calcium, Continuous Spectra, Hydrogen, Potassium, Stellar Spectra, Astrophysics, CA II EMISSION, INSTRUMENTS, STARS: CHROMOSPHERES},
         year = 1991,
        month = may,
       volume = {76},
        pages = {383},
          doi = {10.1086/191572},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991ApJS...76..383D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2016A&A...587A.150U,
       author = {{Usoskin}, I.~G. and {Gallet}, Y. and {Lopes}, F. and {Kovaltsov}, G.~A. and {Hulot}, G.},
        title = "{Solar activity during the Holocene: the Hallstatt cycle and its consequence for grand minima and maxima}",
      journal = {\aap},
     keywords = {Sun: activity, solar-terrestrial relations, Astrophysics - Solar and Stellar Astrophysics, Physics - Geophysics},
         year = 2016,
        month = mar,
       volume = {587},
          eid = {A150},
        pages = {A150},
          doi = {10.1051/0004-6361/201527295},
archivePrefix = {arXiv},
       eprint = {1602.02483},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...587A.150U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998MNRAS.297.1123K,
       author = {{Knobloch}, E. and {Tobias}, S.~M. and {Weiss}, N.~O.},
        title = "{Modulation and symmetry changes in stellar dynamos}",
      journal = {\mnras},
     keywords = {CHAOS, MHD, SUN: MAGNETIC FIELDS, SUNSPOTS, STARS: MAGNETIC FIELDS},
         year = 1998,
        month = jul,
       volume = {297},
       number = {4},
        pages = {1123-1138},
          doi = {10.1046/j.1365-8711.1998.01572.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998MNRAS.297.1123K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...729...80H,
       author = {{Hathaway}, David H. and {Rightmire}, Lisa},
        title = "{Variations in the Axisymmetric Transport of Magnetic Elements on the Sun: 1996-2010}",
      journal = {\apj},
     keywords = {Sun: dynamo, Sun: rotation, Sun: surface magnetism, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = mar,
       volume = {729},
       number = {2},
          eid = {80},
        pages = {80},
          doi = {10.1088/0004-637X/729/2/80},
archivePrefix = {arXiv},
       eprint = {1010.1242},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...729...80H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2015Sci...347.1333C,
       author = {{Cameron}, Robert and {Sch{\"u}ssler}, Manfred},
        title = "{The crucial role of surface magnetic fields for the solar dynamo}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = mar,
       volume = {347},
       number = {6228},
        pages = {1333-1335},
          doi = {10.1126/science.1261470},
archivePrefix = {arXiv},
       eprint = {1503.08469},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015Sci...347.1333C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018A&A...618A..89S,
       author = {{Sch{\"u}ssler}, M. and {Cameron}, R.~H.},
        title = "{Origin of the hemispheric asymmetry of solar activity}",
      journal = {\aap},
     keywords = {Sun: activity, Sun: magnetic fields, dynamo, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = oct,
       volume = {618},
          eid = {A89},
        pages = {A89},
          doi = {10.1051/0004-6361/201833532},
archivePrefix = {arXiv},
       eprint = {1807.10061},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...618A..89S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994SoPh..150....1S,
       author = {{Schrijver}, C.~J. and {Harvey}, K.~L.},
        title = "{The Photospheric Magnetic Flux Budget}",
      journal = {\solphys},
     keywords = {Emission Spectra, Faculae, Line Spectra, Magnetic Flux, Photosphere, Solar Flux, Solar Flux Density, Solar Interior, Solar Magnetic Field, Solar Spectra, Sunspots, Magnetic Signatures, Mathematical Models, Stellar Magnetic Fields, Stellar Models, Synoptic Measurement, Zeeman Effect, Solar Physics},
         year = 1994,
        month = mar,
       volume = {150},
        pages = {1},
          doi = {10.1007/BF00712873},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994SoPh..150....1S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2018A&A...609A..56C,
       author = {{Cameron}, R.~H. and {Duvall}, T.~L. and {Sch{\"u}ssler}, M. and {Schunker}, H.},
        title = "{Observing and modeling the poloidal and toroidal fields of the solar dynamo}",
      journal = {\aap},
     keywords = {Sun: magnetic fields, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = jan,
       volume = {609},
          eid = {A56},
        pages = {A56},
          doi = {10.1051/0004-6361/201731481},
archivePrefix = {arXiv},
       eprint = {1710.07126},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...609A..56C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Baliunas1995ApJ...438..269B,
       author = {{Baliunas}, S.~L. and {Donahue}, R.~A. and {Soon}, W.~H. and {Horne}, J.~H. and {Frazer}, J. and {Woodard-Eklund}, L. and {Bradford}, M. and {Rao}, L.~M. and {Wilson}, O.~C. and {Zhang}, Q. and {Bennett}, W. and {Briggs}, J. and {Carroll}, S.~M. and {Duncan}, D.~K. and {Figueroa}, D. and {Lanning}, H.~H. and {Misch}, T. and {Mueller}, J. and {Noyes}, R.~W. and {Poppe}, D. and {Porter}, A.~C. and {Robinson}, C.~R. and {Russell}, J. and {Shelton}, J.~C. and {Soyumer}, T. and {Vaughan}, A.~H. and {Whitney}, J.~H.},
        title = "{Chromospheric Variations in Main-Sequence Stars. II.}",
      journal = {\apj},
     keywords = {Chromosphere, Emission Spectra, Main Sequence Stars, Stellar Activity, Stellar Evolution, Variations, Calcium, Flux Density, H Lines, K Lines, Stellar Magnetic Fields, Stellar Rotation, Astrophysics, STARS: ACTIVITY, STARS: CHROMOSPHERES, STARS: LATE-TYPE, STARS: ROTATION},
         year = 1995,
        month = jan,
       volume = {438},
        pages = {269},
          doi = {10.1086/175072},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...438..269B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Metcalfe2013ApJ...763L..26M,
       author = {{Metcalfe}, T.~S. and {Buccino}, A.~P. and {Brown}, B.~P. and {Mathur}, S. and {Soderblom}, D.~R. and {Henry}, T.~J. and {Mauas}, P.~J.~D. and {Petrucci}, R. and {Hall}, J.~C. and {Basu}, S.},
        title = "{Magnetic Activity Cycles in the Exoplanet Host Star epsilon Eridani}",
      journal = {\apjl},
     keywords = {stars: activity, stars: chromospheres, stars: individual: HD 22049, surveys, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = feb,
       volume = {763},
       number = {2},
          eid = {L26},
        pages = {L26},
          doi = {10.1088/2041-8205/763/2/L26},
archivePrefix = {arXiv},
       eprint = {1212.4425},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...763L..26M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{BoroSaikia-Sindex-2018A&A...616A.108B,
       author = {{Boro Saikia}, S. and {Marvin}, C.~J. and {Jeffers}, S.~V. and {Reiners}, A. and {Cameron}, R. and {Marsden}, S.~C. and {Petit}, P. and {Warnecke}, J. and {Yadav}, A.~P.},
        title = "{Chromospheric activity catalogue of 4454 cool stars. Questioning the active branch of stellar activity cycles}",
      journal = {\aap},
     keywords = {stars: chromospheres, stars: activity, stars: solar-type, stars: late-type, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = aug,
       volume = {616},
          eid = {A108},
        pages = {A108},
          doi = {10.1051/0004-6361/201629518},
archivePrefix = {arXiv},
       eprint = {1803.11123},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...616A.108B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1969ApJ...156....1L,
       author = {{Leighton}, Robert B.},
        title = "{A Magneto-Kinematic Model of the Solar Cycle}",
      journal = {\apj},
         year = 1969,
        month = apr,
       volume = {156},
        pages = {1},
          doi = {10.1086/149943},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1969ApJ...156....1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1961ApJ...133..572B,
       author = {{Babcock}, H.~W.},
        title = "{The Topology of the Sun's Magnetic Field and the 22-YEAR Cycle.}",
      journal = {\apj},
         year = 1961,
        month = mar,
       volume = {133},
        pages = {572},
          doi = {10.1086/147060},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1961ApJ...133..572B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994SoPh..154..275G,
       author = {{Garcia}, Howard A.},
        title = "{Temperature and Emission Measure from Goes Soft X-Ray Measurements}",
      journal = {\solphys},
     keywords = {Data Processing, Emission Spectra, Error Analysis, Solar Spectra, Solar Temperature, Solar X-Rays, Stellar Models, X Ray Astronomy, X Ray Spectra, Astronomical Spectroscopy, Calibrating, Data Reduction, Goes Satellites, Instrument Errors, Mathematical Models, Synchronous Meteorological Satellite, X Ray Spectroscopy, Solar Physics},
         year = 1994,
        month = oct,
       volume = {154},
       number = {2},
        pages = {275-308},
          doi = {10.1007/BF00681100},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994SoPh..154..275G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017ApJ...835...25E,
       author = {{Egeland}, Ricky and {Soon}, Willie and {Baliunas}, Sallie and {Hall}, Jeffrey C. and {Pevtsov}, Alexei A. and {Bertello}, Luca},
        title = "{The Mount Wilson Observatory S-index of the Sun}",
      journal = {\apj},
     keywords = {stars: activity, Sun: activity, Sun: chromosphere, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jan,
       volume = {835},
       number = {1},
          eid = {25},
        pages = {25},
          doi = {10.3847/1538-4357/835/1/25},
archivePrefix = {arXiv},
       eprint = {1611.04540},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...835...25E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1844AN.....21..233S,
       author = {{Schwabe}, Heinrich},
        title = "{Sonnenbeobachtungen im Jahre 1843. Von Herrn Hofrath Schwabe in Dessau}",
      journal = {Astronomische Nachrichten},
         year = 1844,
        month = feb,
       volume = {21},
       number = {15},
        pages = {233},
          doi = {10.1002/asna.18440211505},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1844AN.....21..233S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1908ApJ....28..315H,
       author = {{Hale}, George E.},
        title = "{On the Probable Existence of a Magnetic Field in Sun-Spots}",
      journal = {\apj},
         year = 1908,
        month = nov,
       volume = {28},
        pages = {315},
          doi = {10.1086/141602},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1908ApJ....28..315H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Cameron2018A&A...609A..56C,
       author = {{Cameron}, R.~H. and {Duvall}, T.~L. and {Sch{\"u}ssler}, M. and {Schunker}, H.},
        title = "{Observing and modeling the poloidal and toroidal fields of the solar dynamo}",
      journal = {\aap},
     keywords = {Sun: magnetic fields, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = jan,
       volume = {609},
          eid = {A56},
        pages = {A56},
          doi = {10.1051/0004-6361/201731481},
archivePrefix = {arXiv},
       eprint = {1710.07126},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...609A..56C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Coffaro2020A&A...636A..49C,
       author = {{Coffaro}, M. and {Stelzer}, B. and {Orlando}, S. and {Hall}, J. and {Metcalfe}, T.~S. and {Wolter}, U. and {Mittag}, M. and {Sanz-Forcada}, J. and {Schneider}, P.~C. and {Ducci}, L.},
        title = "{An X-ray activity cycle on the young solar-like star ɛ Eridani}",
      journal = {\aap},
     keywords = {X-rays: stars, stars: solar-type, stars: activity, stars: coronae, stars: individual: ɛ Eridani, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = apr,
       volume = {636},
          eid = {A49},
        pages = {A49},
          doi = {10.1051/0004-6361/201936479},
archivePrefix = {arXiv},
       eprint = {2002.11009},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...636A..49C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Jeffers2014A&A...569A..79J,
       author = {{Jeffers}, S.~V. and {Petit}, P. and {Marsden}, S.~C. and {Morin}, J. and {Donati}, J. -F. and {Folsom}, C.~P.},
        title = "{ɛ Eridani: an active K dwarf and a planet hosting star?. The variability of its large-scale magnetic field topology}",
      journal = {\aap},
     keywords = {magnetic fields, stars: activity, stars: magnetic field, starspots},
         year = 2014,
        month = sep,
       volume = {569},
          eid = {A79},
        pages = {A79},
          doi = {10.1051/0004-6361/201423725},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...569A..79J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jeffers2017MNRAS.471L..96J,
       author = {{Jeffers}, S.~V. and {Boro Saikia}, S. and {Barnes}, J.~R. and {Petit}, P. and {Marsden}, S.~C. and {Jardine}, M.~M. and {Vidotto}, A.~A. and {BCool Collaboration}},
        title = "{The relation between stellar magnetic field geometry and chromospheric activity cycles - I. The highly variable field of {\ensuremath{\in}} Eridani at activity minimum}",
      journal = {\mnras},
     keywords = {techniques: polarimetric, stars: activity, stars: individual: {\ensuremath{\in}} Eridani, stars: magnetic field, stars: solar-type, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jul,
       volume = {471},
       number = {1},
        pages = {L96-L100},
          doi = {10.1093/mnrasl/slx097},
archivePrefix = {arXiv},
       eprint = {1710.09227},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.471L..96J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{BoroSaikia2018A&A...620L..11B,
       author = {{Boro Saikia}, S. and {Lueftinger}, T. and {Jeffers}, S.~V. and {Folsom}, C.~P. and {See}, V. and {Petit}, P. and {Marsden}, S.~C. and {Vidotto}, A.~A. and {Morin}, J. and {Reiners}, A. and {Guedel}, M. and {BCool Collaboration}},
        title = "{Direct evidence of a full dipole flip during the magnetic cycle of a sun-like star}",
      journal = {\aap},
     keywords = {stars: magnetic field, stars: solar-type, stars: imaging, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = dec,
       volume = {620},
          eid = {L11},
        pages = {L11},
          doi = {10.1051/0004-6361/201834347},
archivePrefix = {arXiv},
       eprint = {1811.11671},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...620L..11B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{BoroSaikia2016A&A...594A..29B,
       author = {{Boro Saikia}, S. and {Jeffers}, S.~V. and {Morin}, J. and {Petit}, P. and {Folsom}, C.~P. and {Marsden}, S.~C. and {Donati}, J. -F. and {Cameron}, R. and {Hall}, J.~C. and {Perdelwitz}, V. and {Reiners}, A. and {Vidotto}, A.~A.},
        title = "{A solar-like magnetic cycle on the mature K-dwarf 61 Cygni A (HD 201091)}",
      journal = {\aap},
     keywords = {dynamo, stars: activity, stars: chromospheres, stars: magnetic field, stars: solar-type, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = oct,
       volume = {594},
          eid = {A29},
        pages = {A29},
          doi = {10.1051/0004-6361/201628262},
archivePrefix = {arXiv},
       eprint = {1606.01032},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...594A..29B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Usoskin2008LRSP....5....3U,
       author = {{Usoskin}, Ilya G.},
        title = "{A History of Solar Activity over Millennia}",
      journal = {Living Reviews in Solar Physics},
     keywords = {solar activity, paleo-astrophysics, cosmogenic isotope, solar-terrestrial relations, solar physics, long-term reconstructions, solar dynamo, Solar Activity, Sunspot Number, Solar Energetic Particle, Solar Energetic Particle Event, Maunder Minimum, Astrophysics},
         year = 2008,
        month = oct,
       volume = {5},
       number = {1},
          eid = {3},
        pages = {3},
          doi = {10.12942/lrsp-2008-3},
archivePrefix = {arXiv},
       eprint = {0810.3972},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008LRSP....5....3U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


